Pionic Dark Matter

We study a phenomenological model where the lightest dark matter (DM) particles are the pseudo-Goldstone excitations associated with a spontaneously broken symmetry, and transforming linearly with respect to an unbroken group H. For definiteness we take H = SU(N) and assume the Goldstone particles are bosons; in parallel with QCD, we refer to these particles as dark-matter pions. This scenario is in contrast to the common assumption that DM fields transform linearly under the full symmetry of the model. We illustrate the formalism by treating in detail the case of H = SU(2), in particular we calculate all the interactions relevant for the Boltzmann equations, which we solve numerically; we also derive approximate analytic solutions and show their consistency with the numerical results. We then compare the results with the constraints derived from the cold DM and direct detection experiments and derive the corresponding restrictions on the model parameters.

==> mylatex.tex <==
\usepackage{bbm}                                                  
%\usepackage{mathabx}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                             %
%                     EQUATIONS & ETC SHORTHANDS                              %
%                                                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


\newcommand{\nc}{\newcommand}
%
\nc{\beq}{\begin{equation}}  \nc{\eeq}{\end{equation}}
\nc{\bea}{\begin{eqnarray}}  \nc{\eea}{\end{eqnarray}}
\nc{\baa}{\begin{array}}     \nc{\eaa}{\end{array}}
\nc{\bit}{\begin{itemize}}   \nc{\eit}{\end{itemize}}
\nc{\ben}{\begin{enumerate}} \nc{\een}{\end{enumerate}}
\nc{\bce}{\begin{center}}    \nc{\ece}{\end{center}}
\nc{\bpm}{\begin{pmatrix}}   \nc{\epm}{\end{pmatrix}}
\nc{\bvt}{\begin{verbatim}}  \nc{\evt}{\end{verbatim}}
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                             %
%                     DEFINITION OF SOME SYMBOLS                              %
%                                                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\iszero{\hskip -0.30in \parbox[c]{0.42in}{\psfig{figure=iszero.eps,width=0.42in,silent=}}\hskip -0.12in}
%   which requires ~vandalen/phy130a/notes/iszero.eps which I have not copied yet
\def\andit{{\it\&}}
\def\half{\frac12}	%\def\half{{1\over2}}
\def\third{\frac13}	%\def\third{{1\over3}}
\def\quarter{\frac14}	%\def\quarter{{1\over4}}
\def\rii{\sqrt{2}}
\def\to{\rightarrow}
\def\S{\mathhexbox279}
\def\gesim{\gtrsim}
\def\lesim{\lesssim}
%\def\gesim{\,{\raise-3pt\hbox{$\sim$}}\!\!\!\!\!{\raise2pt\hbox{$>$}}\,}
%\def\lesim{\,{\raise-3pt\hbox{$\sim$}}\!\!\!\!\!{\raise2pt\hbox{$<$}}\,}
\def\boldoverdot{\,{\raise6pt\hbox{\bf.}\!\!\!\!\>}}
\def\re{{\bf Re}}
\def\im{{\bf Im}}
\def\ie{{\it i.e.}}
\def\eg{{\it eg.}}
\def\cf{{\it cf.}\ }
\def\ibid{{\it ibid.}\ }
\def\etal{{\it et al.}}
\def\then{{\quad\Rightarrow\quad}}
\def\acal{{\cal A}}
\def\bcal{{\cal B}}
\def\ccal{{\cal C}}
\def\dcal{{\cal D}}
\def\ecal{{\cal E}}
\def\fcal{{\cal F}}
\def\gcal{{\cal G}}
\def\hcal{{\cal H}}
\def\ical{{\cal I}}
\def\jcal{{\cal J}}
\def\kcal{{\cal K}}
\def\lcal{{\cal L}}
\def\mcal{{\cal M}}
\def\ncal{{\cal N}}
\def\ocal{{\cal O}}
\def\pcal{{\cal P}}
\def\qcal{{\cal Q}}
\def\rcal{{\cal R}}
\def\scal{{\cal S}}
\def\tcal{{\cal T}}
\def\ucal{{\cal U}}
\def\vcal{{\cal V}}
\def\wcal{{\cal W}}
\def\xcal{{\cal X}}
\def\ycal{{\cal Y}}
\def\zcal{{\cal Z}}
%
\def\aa{{\bf a}}
\def\bb{{\bf b}}
\def\cc{{\bf c}}
\def\dd{{\bf d}}
\def\ee{{\bf e}}
\def\ff{{\bf f}}
\def\ggg{{\bf g}}
\def\hh{{\bf h}}
\def\ii{{\bf i}}
\def\jj{{\bf j}}
\def\kk{{\bf k}}
\def\lll{{\bf l}}
\def\mm{{\bf m}}
\def\nn{{\bf n}}
\def\oo{{\bf o}}
\def\pp{{\bf p}}
\def\qq{{\bf q}}
\def\rr{{\bf r}}
\def\ss{{\bf s}}
\def\ttt{{\bf t}}
\def\uu{{\bf u}}
\def\vv{{\bf v}}
\def\ww{{\bf w}}
\def\xx{{\bf x}}
\def\yy{{\bf y}}
\def\zz{{\bf z}}
%
\def\AA{{\bf A}}
\def\BB{{\bf B}}
\def\CC{{\bf C}}
\def\DD{{\bf D}}
\def\EE{{\bf E}}
\def\FF{{\bf F}}
\def\GG{{\bf G}}
\def\HH{{\bf H}}
\def\II{{\bf I}}
\def\JJ{{\bf J}}
\def\KK{{\bf K}}
\def\LL{{\bf L}}
\def\MM{{\bf M}}
\def\NN{{\bf N}}
\def\OO{{\bf O}}
\def\PP{{\bf P}}
\def\QQ{{\bf Q}}
\def\RR{{\bf R}}
\def\SS{{\bf S}}
\def\TT{{\bf T}}
\def\UU{{\bf U}}
\def\VV{{\bf V}}
\def\WW{{\bf W}}
\def\XX{{\bf X}}
\def\YY{{\bf Y}}
\def\ZZ{{\bf Z}}
%
\def\aBB{{\mathbbm A}}
\def\bBB{{\mathbbm B}}%\def\bBB{ \hbox{{\mysmallii I}}\!\hbox{{\mysmallii B}} }
\def\cBB{{\mathbbm C}}
\def\dBB{{\mathbbm D}}
\def\eBB{{\mathbbm E}}
\def\fBB{{\mathbbm F}}
\def\gBB{{\mathbbm G}}
\def\hBB{{\mathbbm H}}
\def\iBB{{\mathbbm I}}%\def\iBB{ \hbox{{\mysmallii I}}\!\hbox{{\mysmallii I}} }
\def\jBB{{\mathbbm J}}
\def\kBB{{\mathbbm K}}
\def\lBB{{\mathbbm L}}
\def\mBB{{\mathbbm M}}%\def\mBB{ \hbox{{\mysmallii I}}\!\hbox{{\mysmallii M}} }
%
\def\nBB{{\mathbbm N}}
\def\oBB{{\mathbbm O}}
\def\pBB{{\mathbbm P}}%\def\pBB{ \hbox{{\mysmallii I}}\!\hbox{{\mysmallii P}} }
\def\qBB{{\mathbbm Q}}
\def\rBB{{\mathbbm R}}%\def\rBB{ \hbox{{\mysmallii I}}\!\hbox{{\mysmallii R}} }
\def\sBB{{\mathbbm S}}
\def\tBB{{\mathbbm T}}
\def\uBB{{\mathbbm U}}
\def\vBB{{\mathbbm V}}
\def\wBB{{\mathbbm W}}
\def\xBB{{\mathbbm X}}
\def\yBB{{\mathbbm Y}}
\def\zBB{{\mathbbm Z}}
%
\def\mati{{\mathbbm1}}

%
\usepackage{bm}
% ON THE RIGHT I HAVE THE OLD DEFINITIONS
%
\def\alpbf{{\bm\alpha}}		%	\def\alpbf{{\pmb{$\alpha$}}}
\def\betbf{{\bm\beta}}		%	\def\betbf{{\pmb{$\beta$}}}
\def\gambf{{\bm\gamma}}		%	\def\gambf{{\pmb{$\gamma$}}}
\def\delbf{{\bm\delta}}		%	\def\delbf{{\pmb{$\delta$}}}
\def\epsbf{{\bm\epsilon}}	%	\def\epsbf{{\pmb{$\epsilon$}}}
\def\varepsbf{{\bm\varepsilon}}	%	\def\varepsbf{{\pmb{$\varepsilon$}}}
\def\zetbf{{\bm\zeta}}		%	\def\zetbf{{\pmb{$\zeta$}}}
\def\etabf{{\bm\eta}}		%	\def\etabf{{\pmb{$\eta$}}}
\def\thebf{{\bm\theta}}		%	\def\thebf{{\pmb{$\theta$}}}
\def\varthebf{{\bm\vartheta}}	%	\def\varthebf{{\pmb{$\vartheta$}}}
\def\iotbf{{\bm\iota}}		%	\def\iotbf{{\pmb{$\iota$}}}
\def\kapbf{{\bm\kappa}}		%	\def\kapbf{{\pmb{$\kappa$}}}
\def\lambf{{\bm\lambda}}	%	\def\lambf{{\pmb{$\lambda$}}}
\def\mubf{{\bm\mu}}		%	\def\mubf{{\pmb{$\mu$}}}
\def\nubf{{\bm\nu}}		%	\def\nubf{{\pmb{$\nu$}}}
\def\xibf{{\bm\xi}}		%	\def\xibf{{\pmb{$\xi$}}}
% no omicron, apparently
\def\pibf{{\bm\pi}}		%	\def\pibf{{\pmb{$\pi$}}}
\def\varpibf{{\bm\varpi}}	%	\def\varpibf{{\pmb{$\varpi$}}}
\def\rhobf{{\bm\rho}}		%	\def\rhobf{{\pmb{$\rho$}}}
\def\sigbf{{\bm\sigma}}		%	\def\sigbf{{\pmb{$\sigma$}}}
\def\taubf{{\bm\tau}}		%	\def\taubf{{\pmb{$\tau$}}}
\def\upsbf{{\bm\upsilon}}	%	\def\upsbf{{\pmb{$\upsilon$}}}
\def\phibf{{\bm\phi}}		%	\def\phibf{{\pmb{$\phi$}}}
\def\varphibf{{\bm\varphi}}	%	\def\varphibf{{\pmb{$\varphi$}}}
\def\chibf{{\bm\chi}}		%	\def\chibf{{\pmb{$\chi$}}}
\def\psibf{{\bm\psi}}		%	\def\psibf{{\pmb{$\psi$}}}
\def\omebf{{\bm\omega}}		%	\def\omebf{{\pmb{$\omega$}}}
%
\def\Gambf{{\bm\Gamma}}		%	\def\Gambf{{\pmb{$\Gamma$}}}
\def\Delbf{{\bm\Delta}}		%	\def\Delbf{{\pmb{$\Delta$}}}
\def\Thebf{{\bm\Theta}}		%	\def\Thebf{{\pmb{$\Theta$}}}
\def\Lambf{{\bm\Lambda}}	%	\def\Lambf{{\pmb{$\Lambda$}}}
\def\Xibf{{\bm\Xi}}		%	\def\Xibf{{\pmb{$\Xi$}}}
\def\Pibf{{\bm\Pi}}		%	\def\Pibf{{\pmb{$\Pi$}}}
\def\Sigbf{{\bm\Sigma}}		%	\def\Sigbf{{\pmb{$\Sigma$}}}
\def\Upsbf{{\bm\Upsilon}}	%	\def\Upsbf{{\pmb{$\Upsilon$}}}
\def\Phibf{{\bm\Phi}}		%	\def\Phibf{{\pmb{$\Phi$}}}
\def\Psibf{{\bm\Psi}}		%	\def\Psibf{{\pmb{$\Psi$}}}
\def\Omebf{{\bm\Omega}}		%	\def\Omebf{{\pmb{$\Omega$}}}
%
\def\ssb{spontaneous symmetry breaking}
\def\vev{vacuum expectation value}
\def\irrep{irreducible representation}
\def\lhs{left hand side\ }
\def\rhs{right hand side\ }
\def\Ssb{Spontaneous symmetry breaking\ }
\def\Vev{Vacuum expectation value}
\def\Irrep{Irreducible representation}
\def\Lhs{Left hand side\ }
\def\Rhs{Right hand side\ }
\def\tr{ \hbox{tr}}
\def\det{\hbox{det}}
\def\Tr{ \hbox{Tr}}
\def\Det{\hbox{Det}}
\def\diag{\hbox{\diag}}
\def\sm{Standard Model}
%
\def\ev{\hbox{eV}}
\def\kev{\hbox{keV}}
\def\mev{\hbox{MeV}}
\def\gev{\hbox{GeV}}
\def\tev{\hbox{TeV}}
\def\milm{\hbox{mm}}
\def\cm{\hbox{cm}}
\def\m{\hbox{m}}
\def\km{\hbox{km}}
\def\gr{\hbox{gr}}
\def\kg{\hbox{kg}}
%
\def\STOP{\medskip\hrule\smallskip\par\centerline
                  {\large\bf ** STOPPED HERE ** }\smallskip\hrule\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                             %
%                     DEFINITION OF SOME MACROS                               %
%                                                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\pquad{{\phantom{\quad}}}
%
\def\noteeye{{{$(\!(\subset\!\!\!\bullet\!\!\!\supset)\!)\star\star\star$}}}
\def\eyenote{{{$\star\star\star(\!(\subset\!\!\!\bullet\!\!\!\supset)\!)$}}}
\def\note#1{{\bf\noteeye\nobreak{\Large\sc#1}\eyenote } }
%
\def\vevof#1{\left\langle #1 \right\rangle}
\def\ket#1{\left| #1 \right\rangle}
\def\bra#1{\left\langle #1 \right|}
%
\def\doubleundertext#1{
{\undertext{\vphantom{y}#1}}\par\nobreak\vskip-\the\baselineskip\vskip4pt%
\undertext{\hbox to 2in{}}}
%
\def\inbox#1{\vbox{\hrule\hbox{\vrule\kern5pt
     \vbox{\kern5pt#1\kern5pt}\kern5pt\vrule}\hrule}}
%
\def\sqr#1#2{{\vcenter{\hrule height.#2pt
      \hbox{\vrule width.#2pt height#1pt \kern#1pt
         \vrule width.#2pt}
      \hrule height.#2pt}}}
\def\square{\mathchoice\sqr56\sqr56\sqr{2.1}3\sqr{1.5}3}
%
\def\today{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}
%
\def\pmb#1{\setbox0=\hbox{#1}%
  \kern-.025em\copy0\kern-\wd0
  \kern.05em\copy0\kern-\wd0
  \kern-.025em\raise.0433em\box0 }

\def\pmbb#1{\setbox0=\hbox{#1}%
  \kern-.02em\copy0\kern-\wd0
  \kern.04em\copy0\kern-\wd0
  \kern-.02em\raise.03464em\box0 }
%
\def\up#1{^{\left( #1 \right) }}
%
\def\lowti#1{_{{\rm #1 }}}
%
\def\inv#1{\frac1{#1}}
%
% \def\deriva#1#2#3{\left({\partial #1\over\partial #2}\right)_{#3}}
\def\deriva#1#2#3{\left(\frac{\partial #1}{\partial #2}\right)_{#3}}
%
\def\su#1{{SU(#1)}}
\def\ui{U(1)}
%
\def\antes{}
\def\despues{.}
%
\def\dss{ {}^2 }
% which stands for ``double superscript square''
%
\def\sumprime_#1{\setbox0=\hbox{$\scriptstyle{#1}$}
  \setbox2=\hbox{$\displaystyle{\sum}$}
  \setbox4=\hbox{${}'\mathsurround=0pt$}
  \dimen0=.5\wd0 \advance\dimen0 by-.5\wd2
  \ifdim\dimen0>0pt
  \ifdim\dimen0>\wd4 \kern\wd4 \else\kern\dimen0\fi\fi
\mathop{{\sum}'}_{\kern-\wd4 #1}}
%
\def\dodraft#1{
\special{!userdict begin /bop-hook{gsave 200 30 translate
65 rotate /Times-Roman findfont 216 scalefont setfont 
0 0 moveto .8 setgray (DRAFT) show grestore
/Times-Roman findfont 50 scalefont setfont 
50 100 translate
65 rotate
0 0 moveto .8 setgray ([#1: \today]) show grestore}def end}
\typeout{}
\typeout{**************|||||||||******************}
\typeout{}
\typeout{Paper: #1 (DRAFT)}
\typeout{}
\typeout{**************|||||||||******************}
\typeout{}
\typeout{}
}
%
\def\putnote#1#2{
\special{!userdict begin /bop-hook{gsave 200 30 translate
65 rotate /Times-Roman findfont 216 scalefont setfont 
0 0 moveto 1 setgray (#1) show grestore
/Times-Roman findfont 50 scalefont setfont 
50 100 translate
65 rotate
0 0 moveto .99 setgray ([#2: \today]) show grestore}def end}
}
%
%\newcounter{problem}[section]
%\def\clearprob{\setcounter{problem}{0}}
%\def\prob{\addtocounter{problem}{1} 
%            {\par\medskip $\triangleright$\ \underline{{\sl Problem}}\ 
%                \thesection.\theproblem.\ }} 
%
%\def\clearsect{\setcounter{section}{0}}
%
%\def\clearchap{\setcounter{chapter}{0}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                             %
%                     DEFINITION OF SOME FONTS                                %
%                                                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\font\sanserh=cmssq8 scaled\magstep half
\font\sanser=cmssq8
\font\sanseru=cmssq8 scaled\magstep1 % (this is an old definition)
\font\sanserd=cmssq8 scaled\magstep2 % (this is an old definition)
\font\sanseri=cmssq8 scaled\magstep1
\font\sanserii=cmssq8 scaled\magstep2
\font\sanseriii=cmssq8 scaled\magstep3
\font\sanseriv=cmssq8 scaled\magstep4
\font\sanserv=cmssq8 scaled\magstep5
%
\font\tyt=cmtt10
\font\tyti=cmtt10 scaled\magstep1
\font\tytii=cmtt10 scaled\magstep2
\font\tytiii=cmtt10 scaled\magstep3
\font\tytiv=cmtt10 scaled\magstep4
\font\tytv=cmtt10 scaled\magstep5
%
\font\slanti=cmsl10 scaled\magstep1
\font\slantii=cmsl10 scaled\magstep2
\font\slantiii=cmsl10 scaled\magstep3
\font\slantiv=cmsl10 scaled\magstep4
\font\slantv=cmsl10 scaled\magstep5
%
\font\bigboldi=cmbx10 scaled\magstep1
\font\bigboldii=cmbx10 scaled\magstep2
\font\bigboldiii=cmbx10 scaled\magstep3
\font\bigboldiv=cmbx10 scaled\magstep4
\font\bigboldv=cmbx10 scaled\magstep5
%
\font\mysmall=cmr8
\font\mysmalli=cmr8 scaled\magstep1
\font\mysmallii=cmr8 scaled\magstep2
\font\mysmalliii=cmr8 scaled\magstep3
\font\mysmalliv=cmr8 scaled\magstep4
\font\mysmallv=cmr8 scaled\magstep5
%
\font\ital=cmti10
\font\itali=cmti10 scaled\magstep1
\font\italii=cmti10 scaled\magstep2
\font\italiii=cmti10 scaled\magstep3
\font\italiv=cmti10 scaled\magstep4
\font\italv=cmti10 scaled\magstep5
%
\font\smallit=cmmi7
\font\smalliti=cmmi7 scaled\magstep1
\font\smallitii=cmmi7 scaled\magstep2
%
\font\rmi=cmr10 scaled\magstep1
\font\rmii=cmr10 scaled\magstep2
\font\rmiii=cmr10 scaled\magstep3
\font\rmiv=cmr10 scaled\magstep4
\font\rmv=cmr10 scaled\magstep5
\font\eightrm=cmr8


